EM for Mixture of Linear Regression with Clustered Data

Modern data-driven and distributed learning frameworks deal with diverse massive data generated by clients spread across heterogeneous environments. Indeed, data heterogeneity is a major bottleneck in scaling up many distributed learning paradigms. In many settings however, heterogeneous data may be generated in clusters with shared structures, as is the case in several applications such as federated learning where a common latent variable governs the distribution of all the samples generated by a client. It is therefore natural to ask how the underlying clustered structures in distributed data can be exploited to improve learning schemes. In this paper, we tackle this question in the special case of estimating $d$-dimensional parameters of a two-component mixture of linear regressions problem where each of $m$ nodes generates $n$ samples with a shared latent variable. We employ the well-known Expectation-Maximization (EM) method to estimate the maximum likelihood parameters from $m$ batches of dependent samples each containing $n$ measurements. Discarding the clustered structure in the mixture model, EM is known to require $O(\log(mn/d))$ iterations to reach the statistical accuracy of $O(\sqrt{d/(mn)})$. In contrast, we show that if initialized properly, EM on the structured data requires only $O(1)$ iterations to reach the same statistical accuracy, as long as $m$ grows up as $e^{o(n)}$. Our analysis establishes and combines novel asymptotic optimization and generalization guarantees for population and empirical EM with dependent samples, which may be of independent interest.

==> 3-proofs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Proposition \ref{prop: population EM}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%
\begin{align}
    f_{\theta} (x,y)
    &=
    \int  f_{\theta} (x,y,\xi) \mathrm{d} \xi \\
    &=
    \Prob[\xi = -1] f_{\theta} (x,y | \xi=-1) + \Prob[\xi = +1] f_{\theta} (x,y | \xi=+1)\\
    &=
    \frac{1}{2} \left( \frac{1}{2 \pi \sigma^2} \right)^{n/2} f(x) 
    \left\{ 
    \exp\left( - \frac{1}{2\sigma^2} \sum_{i=1}^{n} \left( y_i - \langle x_i, \theta \rangle \right)^2\right)
    +
    \exp\left( - \frac{1}{2\sigma^2} \sum_{i=1}^{n} \left( y_i + \langle x_i, \theta \rangle \right)^2\right)
    \right\} \\
    &=
    \frac{1}{2} \left( \frac{1}{2 \pi \sigma^2} \right)^{n/2} f(x) 
    \exp\left(  - \frac{1}{2\sigma^2} \sum_{i=1}^{n} y_i^2 \right)
    \exp\left(  - \frac{1}{2\sigma^2} \sum_{i=1}^{n} \langle x_i , \theta \rangle^2 \right) \\
    &\quad \times
    \left\{ 
    \exp\left( - \frac{1}{\sigma^2} \sum_{i=1}^{n} \langle x_i, \theta \rangle y_i \right)
    +
    \exp\left( \frac{1}{\sigma^2} \sum_{i=1}^{n} \langle x_i, \theta \rangle y_i\right)
    \right\} 
\end{align}
%%%%
%%%%
\begin{align}
    Q(\theta' | \theta)
    =
    \int_{(x,y)} \left( \int_{\xi} f_{\theta} (\xi | x,y) \ln\left( f_{\theta'} (x,y,\xi) \right) \mathrm{d} \xi \right) f_{\theta^*}(x,y) \mathrm{d}x \mathrm{d}y
\end{align}
%%%%
Let us define
%%%%
\begin{align}
    \hat{Q}(\theta' | \theta)
    =
    \int_{\xi} f_{\theta} (\xi | x,y) \ln\left( f_{\theta'} (x,y,\xi) \right) \mathrm{d} \xi
\end{align}
%%%%
Therefore, 
%%%%
\begin{align}
    Q(\theta' | \theta)
    =
    \E_{(x,y)} [\hat{Q}(\theta' | \theta)],
\end{align}
%%%%
where in above $x = (x_1, \cdots, x_n)$, $y = (y_1,\cdots,y_n)^\top$, $x_i \overset{\text{i.i.d.}}{\sim} \ccalN(0,I)$, $y_i = \xi \langle x_i, \theta^* \rangle + \epsilon_i$, $\xi \sim \ccalU\{-1,+1\}$ and $\epsilon_i \overset{\text{i.i.d.}}{\sim} \ccalN(0,\sigma^2)$.
%%%%
\begin{align}
    Q(\theta' | \theta)
    =
    - \frac{n}{2\sigma^2} \Vert \theta' \Vert^2
    +
    {\theta'}^{\top}
    \E_{(X,Y)}\left[ \frac{1}{{\color{red}2}\sigma^2} \sum_{i} X_i Y_i \tanh\left( \frac{1}{\sigma^2} \sum_i \langle X_i, \theta\rangle Y_i \right) \right]
    +
    \text{constants},
\end{align}
%%%%
Therefore, $Q(\cdot | \theta^*)$ is $\lambda$--strongly concave with $\lambda = n/\sigma^2$.
%%%%
\begin{align}
    \gr Q(\theta' | \theta)
    =
    - \frac{n}{\sigma^2} \theta' 
    +
    \E_{(X,Y)}\left[ \frac{1}{{\color{red}2}\sigma^2} \sum_{i} X_i Y_i \tanh\left( \frac{1}{\sigma^2} \sum_i \langle X_i, \theta\rangle Y_i \right) \right],
\end{align}
%%%%
We can put $\gr Q(\theta' | \theta) = 0$ to find $M(\theta)$.
%%%%
\begin{align}
    M(\theta)
    &\coloneqq
    \argmax_{\theta'} Q(\theta' | \theta)\\
    &=
    \E_{\substack{X_1,\cdots, X_n \overset{\text{i.i.d.}}{\sim} \ccalN(0,I) \\
    Y_1,\cdots,Y_n | X_1,\cdots,X_n \sim \ccalN(\xi \langle X_i, \theta^* \rangle, \sigma^2)}}
    \left[ \frac{1}{n} \tanh\left( \frac{1}{\sigma^2} \sum_i \langle X_i, \theta\rangle Y_i \right) \sum_{i} X_i Y_i \right]\\
    &=
    \frac{1}{2} 
    \E_{\substack{X_1,\cdots, X_n \overset{\text{i.i.d.}}{\sim} \ccalN(0,I) \\
    Y_1,\cdots,Y_n | X_1,\cdots,X_n \sim \ccalN(- \langle X_i, \theta^* \rangle, \sigma^2)}}
    \left[ \frac{1}{n} \tanh\left( \frac{1}{\sigma^2} \sum_i \langle X_i, \theta\rangle Y_i \right) \sum_{i} X_i Y_i \right]\\
    &\quad +
    \frac{1}{2} 
    \E_{\substack{X_1,\cdots, X_n \overset{\text{i.i.d.}}{\sim} \ccalN(0,I) \\
    Y_1,\cdots,Y_n | X_1,\cdots,X_n \sim \ccalN( \langle X_i, \theta^* \rangle, \sigma^2)}}
    \left[ \frac{1}{n} \tanh\left( \frac{1}{\sigma^2} \sum_i \langle X_i, \theta\rangle Y_i \right) \sum_{i} X_i Y_i \right] \\
    &=
    \E_{\substack{X_1,\cdots, X_n \overset{\text{i.i.d.}}{\sim} \ccalN(0,I) \\
    Y_1,\cdots,Y_n | X_1,\cdots,X_n \overset{\text{i.i.d.}}{\sim} \ccalN( \langle X_i, \theta^* \rangle, \sigma^2)}}
    \left[ \frac{1}{n} \tanh\left( \frac{1}{\sigma^2} \sum_i \langle X_i, \theta\rangle Y_i \right) \sum_{i} X_i Y_i \right] \\
    &=
    \E_{\substack{X_1,\cdots, X_n \overset{\text{i.i.d.}}{\sim} \ccalN(0,I) \\
    Y_1,\cdots,Y_n | X_1,\cdots,X_n \overset{\text{i.i.d.}}{\sim} \ccalN( \langle X_i, \theta^* \rangle, \sigma^2)}}
    \left[ \tanh\left( \frac{1}{\sigma^2} \sum_i \langle X_i, \theta\rangle Y_i \right) X_1 Y_1 \right]
\end{align}
%%%%
To sum up, the population EM update is as follows
%%%%
\begin{align} 
    M(\theta)
    &=
    \E \left[X_1 Y_1 \tanh\left( \frac{1}{\sigma^2} \sum_{i=1}^{n} \langle X_i, \theta\rangle Y_i \right) \right],
\end{align}
%%%%
where the expectation is over i.i.d. $X_i \sim \ccalN(0,I_d)$ and $Y_i = \langle X_i,\theta^* \rangle + \epsilon_i$ with i.i.d. noises $\epsilon_i \sim \ccalN(0, \sigma^2)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Useful Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma} \label{lemma: tanh slope}
For any $x_1, x_2 \geq 0$, we have
%%%%
\begin{align}
    \frac{\tanh(x_2) - \tanh(x_1)}{x_2 - x_1}
    \leq
    \max\{1-\tanh^2(x_1), 1 - \tanh^2(x_2)\}.
\end{align}
%%%%
\end{lemma}
%%%%



%%%%
\begin{lemma} \label{lemma: signal O(n) bound}
Assume that $\| \theta - \theta^*\| \leq \alpha \| \theta^* \|$ for some $0 \leq \alpha < 1$. For any $n$,
%%%%
\begin{align}
    \bigg| \sum_{i=1}^{n} \langle X_i, \theta\rangle \langle X_i, \theta^*\rangle - n \langle \theta, \theta^*\rangle \bigg|
    \leq
    \frac{n}{2} \langle \theta, \theta^*\rangle.
\end{align}
%%%%
with probability at least
%%%%
\begin{align}
    1 -  2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right)
\end{align}
%%%%
\end{lemma}
%%%%
%%%%
\begin{lemma} \label{lemma: noise O(sqrt n) bound}
Assume that $\| \theta - \theta^*\| \leq \alpha \| \theta^* \|$ for some $0 \leq \alpha < 1$. For any $n$,
%%%%
\begin{align}
    \bigg|\sum_{i=1}^{n} \langle X_i, \theta\rangle \epsilon_i \bigg|
    \leq
    \frac{n}{4}\langle \theta, \theta^*\rangle.
\end{align}
%%%%
with probability at least
%%%%
\begin{align}
    1 - 2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right),
\end{align}
%%%%
where $\SNR \coloneqq \| \theta^* \| / \sigma$.

\end{lemma}
%%%%




%%%%
\begin{lemma} \label{lemma: events E1-3}
Assume that $\|\theta - \theta^* \| \leq \alpha \| \theta^* \|$ for some $0 \leq \alpha < 1$ and let $\SNR = \| \theta^* \| / \sigma$ denote the SNR. Then,
%%%%
\begin{align}
    \Prob(\ccalE_1)
    \geq 
    1 - 
    2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right).
\end{align}
%%%%
and
%%%%
\begin{align}
    \Prob(\ccalE_2)
    \geq 
    1 - 
    2 \exp\left( -\frac{n}{8} \right)
    -
    2 \exp\left( -  n \min\left\{ \SNR^2
    ,
    \frac{\SNR}{2} \right\}\right)
\end{align}
%%%%
\end{lemma}
%%%%


%%%%
\begin{definition}[Sub-exponential RV] \label{def: sub-exponential}
A random variable $X$ is said to be sub-exponential with parameter $(\tau^2,b)$ if
%%%%
\begin{align}
    \E \left[\exp \left(\lambda (X - \mu_X) \right) \right] 
    \leq
    \exp\left(\frac{\lambda^2 \tau^2}{2}\right), 
    \quad
    \forall |\lambda| \leq \frac{1}{b}.
\end{align}
%%%%
We denote such RV by $\SubE(\tau^2,b)$.
\end{definition}
%%%%


%%%%
\begin{lemma} \label{lemma: sub-exponential}
Let $X \sim \ccalN(0, I_d)$ be Gaussian. Then, for any $u,v \in \reals^d$, $\langle X, u \rangle \langle X, v \rangle$ is sub-exponential $\SubE(\tau^2,b)$ with
%%%%
\begin{align}
    \tau^2
    =
    4 \| u \|^2 \| v \|^2,
    \quad
    \text{and}
    \quad
    b
    =
    4 \| u \| \| v \|.
\end{align}
%%%%
\end{lemma}
%%%%

%%%%
\begin{theorem} \label{thm: sub-ex concentration}
Let $X_i \sim \SubE(\tau^2, b)$ be iid sub-exponentials. Then,
%%%%
\begin{align}
    \Prob\left( \left| \frac{1}{n} \sum_{i=1}^{n} X_i - \mu_X \right| \geq t \right)
    \leq
    2 \exp\left( -  \min\left\{ \frac{nt^2}{2\tau^2}, \frac{nt}{2b} \right\}\right)
\end{align}
%%%%
\end{theorem}
%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm: FOS}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
We have that
%%%%
\begin{align}
    \norm{ \gr Q(M(\theta)|\theta^*) - \gr Q(M(\theta)|\theta)}
    &=
    \frac{1}{\sigma^2} \norm{ \E \left[ X_1 Y_1 \left(\tanh \left( \frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta\rangle Y_i\right) - \tanh \left(\frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta^*\rangle Y_i \right)\right) \right]} \\
    &=
    \frac{1}{\sigma^2} \max_{\beta: \Vert \beta \Vert = 1} \E \left[ \langle X_1, \beta \rangle Y_1 \left(\tanh \left( \frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta\rangle Y_i\right) - \tanh \left(\frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta^*\rangle Y_i \right)\right)\right] \\
    &\leq
    \frac{1}{\sigma^2} \max_{\beta: \Vert \beta \Vert = 1} \left| \E \left[ \langle X_1, \beta \rangle Y_1 \left(\tanh \left( \frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta\rangle Y_i\right) - \tanh \left(\frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta^*\rangle Y_i \right)\right)\right] \right| \\
    &\leq
    \frac{1}{\sigma^2} \max_{\beta: \Vert \beta \Vert = 1} \sqrt{ \E [ \langle X_1, \beta \rangle^2 Y_1^2]} 
    \sqrt{T_1},
\end{align}
%%%%
where
%%%%
\begin{align}
    T_1
    \coloneqq
    \E \left[ \left(\tanh \left( \frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta\rangle Y_i\right) - \tanh \left(\frac{1}{\sigma^2} \sum_{i} \langle X_i, \theta^*\rangle Y_i \right)\right)^2 \right]
\end{align}
%%%%

\textbf{Bounding $T_1$}

Define the following shorthand notation for any $\theta$
%%%%
\begin{align}
    Z
    \coloneqq
    \sum_{i=1}^{n} X_i Y_i
\end{align}
%%%%

Define event
%%%%
\begin{gather}
    \ccalE = 
    \left\{
    \langle Z, \theta \rangle \geq \frac{n}{4}(1-\alpha)\| \theta^* \|^2
    \text{ and }
    \langle Z, \theta^* \rangle \geq \frac{n}{4}\| \theta^* \|^2
    \text{ and }
    |\langle Z, \theta \rangle - \langle Z, \theta^* \rangle| 
    \leq 
    3n \| \theta^* \| \| \theta - \theta^* \|
    \right\}
\end{gather}
%%%%


\iffalse
Define event
%%%%
\begin{gather}
    \ccalE = 
    \left\{
    Z(\theta) \geq 0
    \text{ and }
    Z(\theta^*) \geq 0
    \text{ and }
    |Z(\theta) - Z(\theta^*)| 
    \leq 
    3n \| \theta^* \| \| \theta - \theta^* \|
    \right\}
\end{gather}
%%%%
\ar{We probably need to change event to
%%%%
\begin{gather}
    \ccalE = 
    \left\{
    \langle Z, \theta \rangle \geq \frac{n}{4}(1-\alpha)\| \theta^* \|^2
    \text{ and }
    \langle Z, \theta^* \rangle \geq \frac{n}{4}\| \theta^* \|^2
    \text{ and }
    |\langle Z, \theta \rangle - \langle Z, \theta^* \rangle| 
    \leq 
    3n \| \theta^* \| \| \theta - \theta^* \|
    \right\}
\end{gather}
%%%%
}
\fi
Now, we can write
%%%%
\begin{align}
    T_1
    &=
    \E \left[ \left(\tanh \left( \frac{1}{\sigma^2} \langle Z, \theta \rangle \right) 
    -
    \tanh \left(\frac{1}{\sigma^2} \langle Z, \theta^* \rangle \right)\right)^2 \right] \\
    &\leq
    \E \left[ \left(\tanh \left( \frac{1}{\sigma^2} \langle Z, \theta \rangle \right) 
    -
    \tanh \left(\frac{1}{\sigma^2} \langle Z, \theta^* \rangle \right)\right)^2 | \ccalE \right] 
    +
    \E \left[ \left(\tanh \left( \frac{1}{\sigma^2} \langle Z, \theta \rangle \right) 
    -
    \tanh \left(\frac{1}{\sigma^2} \langle Z, \theta^* \rangle \right)\right)^2 | \ccalE^c \right] 
    \Prob(\ccalE^c) 
\end{align}
%%%%


%\begin{align*}
%    \| \mathbb E X_1 Y_1 (\tanh (\sum \langle X_i, \theta\rangle Y_i) - \tanh(\sum \langle X_i, \theta^*\rangle Y_i)) \| \leq \gamma \|\theta - \theta^*\|.
%\end{align*}
%Now assume that $\langle \theta, \theta^*\rangle \geq \alpha, \ \|\theta\| \leq c$ for some fixed constants $\alpha, c$. But we know that with high probability
%\begin{align*}
%    \sum \langle X_i, \theta\rangle Y_i = Z\sum \langle X_i, \theta\rangle \langle X_i, \theta^*\rangle = Z(n\langle \theta, \theta^*\rangle + O(\sqrt n)).
%\end{align*}
%%%%
\begin{align}
    \E \left[ \left(\tanh \left( \frac{1}{\sigma^2} \langle Z, \theta \rangle \right) 
    -
    \tanh \left(\frac{1}{\sigma^2} \langle Z, \theta^* \rangle \right)\right)^2 \big| \ccalE \right]
    &=
    \E \left[
    |\frac{1}{\sigma^2} \langle Z, \theta \rangle - \frac{1}{\sigma^2} \langle Z, \theta^* \rangle|^2
    \left(\frac{\tanh \left(\frac{1}{\sigma^2} \langle Z, \theta \rangle \right) 
    -
    \tanh \left(\frac{1}{\sigma^2} \langle Z, \theta^* \rangle\right)}{\frac{1}{\sigma^2} \langle Z, \theta \rangle - \frac{1}{\sigma^2} \langle Z, \theta^* \rangle}\right)^2 \bigg| \ccalE \right] \\
    &\leq
    \frac{1}{\sigma^2} \E \left[
    |\langle Z, \theta \rangle - \langle Z, \theta^* \rangle|^2
    \left(1 - \tanh^2(\min\{\frac{1}{\sigma^2}\langle Z, \theta \rangle, \frac{1}{\sigma^2}\langle Z, \theta^* \rangle\}) \right)^2 \bigg| \ccalE \right] \\
    &\leq
    9 n^2 \frac{\| \theta^* \|^2}{\sigma^2} \| \theta - \theta^* \|^2
    \left(1 - \tanh^2 \left(\frac{n}{4}(1-\alpha) \frac{\| \theta^* \|^2}{\sigma^2} \right)  \right)^2 \\
    &\leq
    144 n^2 \frac{\| \theta^* \|^2}{\sigma^2} \| \theta - \theta^* \|^2
    \exp \left(-n(1-\alpha)\frac{\| \theta^* \|^2}{\sigma^2} \right)
\end{align}
%%%%
Moreover,
%%%%
\begin{align}
    &\quad
    \E \left[ \left(\tanh \left( \frac{1}{\sigma^2} \langle Z, \theta \rangle \right) 
    -
    \tanh \left(\frac{1}{\sigma^2} \langle Z, \theta^* \rangle \right)\right)^2 | \ccalE^c \right] 
    \Prob(\ccalE^c) \\
    &\leq
    4\Prob(\ccalE^c) \\
    &\leq
    8 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right)
    +
    8 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right) \\
    &\quad +
    8 \exp\left( -\frac{n}{8} \right)
    +
    8 \exp\left( -  n \min\left\{ \SNR^2
    ,
    \frac{\SNR}{2} \right\}\right)\\
    &\leq
    \exp(- 2 c_1 n),
\end{align}
%%%%
for a constant $c_1$ depending on $\alpha$ and $\SNR$. Therefore,
%%%%
\begin{align}
    \frac{T_1}{\| \theta - \theta^* \|^2}
    &=
    \frac{1}{\| \theta - \theta^* \|^2}
    \E \left[ \left(\tanh \left( \frac{1}{\sigma^2} \langle Z, \theta \rangle \right) 
    -
    \tanh \left(\frac{1}{\sigma^2} \langle Z, \theta^* \rangle \right)\right)^2 \right] \\
    &\leq
    144  n^2 \frac{\| \theta^* \|^2}{\sigma^2}
    \exp \left(-n(1-\alpha)\frac{\| \theta^* \|^2}{\sigma^2} \right)
    +
    \frac{\exp(- 2 c_1 n)}{\| \theta - \theta^* \|^2} \\
    &\leq
    144 n^2 \frac{\| \theta^* \|^2}{\sigma^2} \exp \left(-n(1-\alpha)\frac{\| \theta^* \|^2}{\sigma^2} \right)  
    +
    \varepsilon^{-2} \exp(- 2 c_1 n)
\end{align}
%%%%
where we assume that $\| \theta - \theta^* \| \geq \varepsilon$. Therefore,
%%%%
\begin{align}
    \frac{\sqrt{T_1}}{\| \theta - \theta^* \|}
    &\leq
    12 n \frac{\| \theta^* \|}{\sigma} \exp \left(-\frac{n}{2} (1-\alpha)\SNR^2 \right)  
    +
    \varepsilon^{-1} \exp(- c_1 n)
\end{align}
%%%%
Also,
%%%%
\begin{align}
    \E [ \langle X_1, \beta \rangle^2 Y_1^2]
    &=
    \E[ \langle X_1, \beta \rangle^2 \langle X_1, \theta^* \rangle^2]
    +
    \E[\langle X_1, \beta \rangle^2 \epsilon_1^2]\\
    &=
    \langle \beta, \theta^* \rangle \beta^\top \E[ \| X_1 \|^2 X_1 X_1^\top] \theta^*
    +
    \sigma^2 \beta^\top \E[X_1 X_1^\top] \beta \\
    &=
    (d+2) \langle \beta, \theta^* \rangle^2 + \sigma^2 \| \beta \|^2
\end{align}
%%%%
which yields that
%%%%
\begin{align}
    \max_{\beta: \Vert \beta \Vert = 1} \sqrt{ \E [ \langle X_1, \beta \rangle^2 Y_1^2]}
    \leq
    \sqrt{d+2} \| \theta^* \| + \sigma.
\end{align}
%%%%
All in all,
%%%%
\begin{align}
    \Vert \gr Q(M(\theta)|\theta^*) - \gr Q(M(\theta)|\theta) \Vert
    \leq
    \gamma \Vert \theta - \theta^* \Vert.
\end{align}
%%%%
where
%%%%
\begin{align}
    \gamma
    &=
    \frac{1}{\sigma^2} \left( 12 n \frac{\| \theta^* \|}{\sigma} \exp \left(-\frac{n}{2} (1-\alpha)\SNR^2\right)  
    +
    \varepsilon^{-1} \exp(- c_1 n) \right)
    \cdot
    \left( \sqrt{d+2} \| \theta^* \| + \sigma \right) \\
    &\leq
    \frac{1}{\sigma^2} \left( \sqrt{d} \| \theta^* \| + \sigma \right)
    \left( n \SNR + \varepsilon^{-1} \right) \exp \left( - c n \right).
\end{align}
%%%%
for a constant $c$ depending on $c_1$, $\alpha$ and $\SNR$ and $n \geq N_0$. Moreover, $Q(\cdot | \theta^*)$ is $\lambda$--strongly concave with $\lambda = n/\sigma^2$. Therefore,
%%%%
\begin{align}
    \frac{\gamma}{\lambda}
    \leq
    \left( \sqrt{d} \| \theta^* \| + \sigma \right)
    \left( \SNR + \frac{1}{n \varepsilon} \right) \exp \left( -c n \right).
\end{align}
%%%%




\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma: signal O(n) bound}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Let us denote signal RVs $S_i \coloneqq \langle X_i, \theta\rangle \langle X_i, \theta^*\rangle$ for each $i \in [n]$ where $\E[S_i] = \langle \theta, \theta^*\rangle$. As shown in Lemma \ref{lemma: sub-exponential}, $S_i$s are iid sub-exponential $S_i \sim \SubE(4 \| \theta \|^2 \| \theta^* \|^2, 4 \| \theta \| \| \theta^* \|)$. This yields that
%%%%
\begin{align} 
    \sum_{i=1}^{n} \langle X_i, \theta\rangle \langle X_i, \theta^*\rangle
    =
    \sum_{i=1}^{n} S_i
    \sim
    \SubE\left(4n \| \theta \|^2 \| \theta^* \|^2, 4\| \theta \| \| \theta^* \| \right)
\end{align}
%%%%
and therefore
%%%%
\begin{align}
    \Prob\left( \left| \sum_{i=1}^{n} S_i - n \langle \theta, \theta^*\rangle \right| \geq nt \right)
    \leq
    2 \exp\left( -  \min\left\{ \frac{nt^2}{8 \| \theta \|^2 \| \theta^* \|^2}, \frac{nt}{8 \| \theta \| \| \theta^* \|} \right\}\right).
\end{align}
%%%%
For a given positive integer $c$, pick $t = \langle \theta, \theta^*\rangle/2$. Then,
%%%%
\begin{align}
    \min\left\{ \frac{nt^2}{8 \| \theta \|^2 \| \theta^* \|^2}, \frac{nt}{8 \| \theta \| \| \theta^* \|} \right\}
    &=
    \min\left\{ \frac{n}{32} \left( \frac{\langle \theta, \theta^*\rangle}{\| \theta \| \| \theta^* \|}\right)^2
    ,
    \frac{n}{16} \left( \frac{\langle \theta, \theta^*\rangle}{\| \theta \| \| \theta^* \|}\right)\right\} \\
    &=
    \frac{n}{32} \left( \frac{\langle \theta, \theta^*\rangle}{\| \theta \| \| \theta^* \|}\right)^2\\
    &\geq
    \frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2
\end{align}
%%%%
 For any $n$ we have that
%%%%
\begin{align}
    \Prob\left( \left| \sum_{i=1}^{n} S_i - n \langle \theta, \theta^*\rangle \right| \leq \frac{n}{2} \langle \theta, \theta^*\rangle \right)
    &\geq
    1 - 2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right).
\end{align}
%%%%
\end{proof}
%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma: tanh slope}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Assume that $x_2 \geq x_1 \geq 0$. Since the function $f(x) \coloneqq \tanh(x)$ is concave in $[0,+\infty)$, we can write
%%%%
\begin{align}
    f(x_2) \leq f(x_1) + (x_2 - x_1) f'(x_1),
\end{align}
%%%%
which yields that
%%%%
\begin{align}
    \frac{\tanh(x_2) - \tanh(x_1)}{x_2 - x_1}
    \leq
    1-\tanh^2(x_1).
\end{align}
%%%%
Similar argument holds for $x_1 \geq x_2 \geq 0$, i.e.,
%%%%
\begin{align}
    \frac{\tanh(x_1) - \tanh(x_2)}{x_1 - x_2}
    \leq
    1-\tanh^2(x_2).
\end{align}
%%%%
\end{proof}
%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma: noise O(sqrt n) bound}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Define $N_i \coloneqq \langle X_i, \theta\rangle \epsilon_i$ where $\langle X_i, \theta\rangle \sim \ccalN(0, \| \theta \|^2)$ and $\epsilon_i \sim \ccalN(0,\sigma^2)$. Since any randomness across the clients, i.e. different $i \in [n]$ is iid, we drop the index $i$ for simplicity of presentation. We know that $N$ is sub-exponential with parameters $\SubE(\tau_N^2, b_N)$. Denote $Z_x \coloneqq \frac{\langle X, \theta\rangle}{\| \theta \|}$ and $Z_{\epsilon} \coloneqq \frac{\epsilon}{\sigma}$. Clearly, $Z_x$ and $Z_{\epsilon}$ are independent standard Gaussian. Moreover,
%%%%
\begin{align} 
    N
    =
    \| \theta \| \sigma Z_x Z_{\epsilon}
    =
    \frac{\| \theta \| \sigma}{4} \left( Z_x + Z_{\epsilon}\right)^2
    -
    \frac{\| \theta \| \sigma}{4} \left( Z_x - Z_{\epsilon}\right)^2.
\end{align}
%%%%
Furthermore, $Z_x + Z_{\epsilon}$ and $Z_x - Z_{\epsilon}$ are zero-mean Gaussian RVs and $\E[(Z_x + Z_{\epsilon})(Z_x - Z_{\epsilon})] = 0$, implying that $Z_x + Z_{\epsilon}$ and $Z_x - Z_{\epsilon}$ are independent. Therefore,
%%%%
\begin{align} 
    \E\left[ \exp\left(\lambda  N \right) \right] 
    &=
    \E\left[ \exp\left(\lambda \| \theta \| \sigma Z_x Z_{\epsilon} \right) \right]\\
    &=
    \E\left[ \exp\left(\frac{\lambda \| \theta \| \sigma}{4} \left( Z_x + Z_{\epsilon}\right)^2
    -
    \frac{\lambda \| \theta \| \sigma}{4} \left( Z_x - Z_{\epsilon}\right)^2 \right) \right]\\
    &=
    \E\left[ \exp\left(\frac{\lambda \| \theta \| \sigma}{4} \left( Z_x + Z_{\epsilon}\right)^2 \right) \right]
    \cdot
    \E\left[ \exp\left(
    - \frac{\lambda \| \theta \| \sigma}{4} \left( Z_x - Z_{\epsilon}\right)^2 \right) \right]\\
    &\leq
    \exp\left( \frac{\lambda^2}{2} \frac{\| \theta \|^2 \sigma^2}{2} \right),
\end{align}
%%%%
for any $|\lambda| \leq \frac{1}{\| \theta \| \sigma}$. This concludes that $N_i \sim \SubE(\| \theta \|^2 \sigma^2/2, \| \theta \| \sigma)$. In above, we use the fact that if $Z \sim \ccalN(0,1)$, then $Z^2 \sim \SubE(4,4)$.

Now, we can write concentration for sum of $N_i$s as follows. We have that
%%%%
\begin{align} 
    \sum_{i=1}^{n} \langle X_i, \theta\rangle \epsilon_i
    =
    \sum_{i=1}^{n} N_i
    \sim
    \SubE\left(\frac{n\| \theta \|^2 \sigma^2}{2}, \| \theta \| \sigma \right) \label{eq: noise SubE}
\end{align}
%%%%
and therefore
%%%%
\begin{align}
    \Prob\left( \left| \sum_{i=1}^{n} N_i \right| \geq nt \right)
    \leq
    2 \exp\left( -  \min\left\{ \frac{nt^2}{\| \theta \|^2 \sigma^2}, \frac{nt}{2\| \theta \| \sigma} \right\}\right).
\end{align}
%%%%
For a given positive integer $c$, pick $t = \langle \theta, \theta^*\rangle/4$. Then,
%%%%
\begin{align}
    \min\left\{ \frac{nt^2}{\| \theta \|^2 \sigma^2}, \frac{nt}{2\| \theta \| \sigma} \right\}
    &=
    \min\left\{ \frac{n}{16} \left( \frac{\langle \theta, \theta^*\rangle}{\| \theta \| \sigma}\right)^2
    ,
    \frac{n}{8} \left( \frac{\langle \theta, \theta^*\rangle}{\| \theta \| \sigma}\right) \right\} \\
    &\geq
    n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}
\end{align}
%%%%

For any $n$ we have that
%%%%
\begin{align}
    \Prob\left( \left| \sum_{i=1}^{n} N_i \right|
    \leq \frac{n}{4}\langle \theta, \theta^*\rangle \right)
    \geq
    1 - 2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right).
\end{align}
%%%%

\end{proof}
%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma: events E1-3}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
From Lemma \ref{lemma: signal O(n) bound} and \ref{lemma: noise O(sqrt n) bound} we know that
%%%%
\begin{gather}
    \bigg| \sum_{i=1}^{n} \langle X_i, \theta\rangle \langle X_i, \theta^*\rangle - n \langle \theta, \theta^*\rangle \bigg|
    \leq
    \frac{n}{2} \langle \theta, \theta^*\rangle,
\end{gather}
%%%%
with probability at least
%%%%
\begin{align}
    1 -  2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right),
\end{align}
%%%%
and
%%%%
\begin{gather}
    \bigg|\sum_{i=1}^{n} \langle X_i, \theta\rangle \epsilon_i \bigg|
    \leq
    \frac{n}{4}\langle \theta, \theta^*\rangle,
\end{gather}
%%%%
with probability at least
%%%%
\begin{align}
    1 - 2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right),
\end{align}
%%%%
Therefore, using union bound, we have that
%%%%
\begin{align} 
    Z(\theta)
    &=
    \sum_{i=1}^{n} \langle X_i, \theta \rangle Y_i\\
    &=
    \sum_{i=1}^{n} \langle X_i, \theta\rangle \langle X_i, \theta^*\rangle 
    +
    \sum_{i=1}^{n} \langle X_i, \theta\rangle \epsilon_i \\
    &\geq
    \frac{n}{4}\langle \theta, \theta^*\rangle \\
    &\geq
    \frac{n}{4}(1-\alpha)\| \theta^* \|^2. \label{eq: Z(theta) positive}
\end{align}
%%%%
with probability at least
%%%%
\begin{align}
    1 - 
    2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right),
\end{align}
%%%%
In above, we used the assumption $\|\theta - \theta^* \| \leq \alpha \| \theta^* \|$ to conclude that $\langle \theta, \theta^*\rangle \geq (1-\alpha)\| \theta^* \|^2$. Moreover, we can put $\alpha = 0$ in \eqref{eq: Z(theta) positive} which yields that for large enough $n$ as characterized in \eqref{eq: condition on n},
%%%%
\begin{align} 
    Z(\theta^*)
    &\geq
    \frac{n}{4} \| \theta^* \|^2.
\end{align}
%%%%
with probability at least
%%%%
\begin{align}
    1 - 
    2 \exp\left( -\frac{n}{32}\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \SNR^2
    ,
    \frac{1}{8} \SNR \right\}\right),
\end{align}
%%%%
 Therefore,
%%%%
\begin{align} 
    \Prob(\ccalE_1) 
    &= 
    \Prob \left(\left\{
    \langle Z, \theta \rangle \geq \frac{n}{4}(1-\alpha)\| \theta^* \|^2
    \text{ and }
    \langle Z, \theta^* \rangle \geq \frac{n}{4}\| \theta^* \|^2
    \right\} \right) \\
    &\geq
    1 - 
    2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right) \\
    &\quad - 
    2 \exp\left( -\frac{n}{32}\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \SNR^2
    ,
    \frac{1}{8} \SNR \right\}\right)
\end{align}
%%%%



    
    
\iffalse
Clearly, if \eqref{eq: Z(theta) positive} holds true, then $Z(\theta) \geq 0$ \emph{and} $Z(\theta^*) \geq 0$ as well. Therefore,
%%%%
\begin{align} 
    \Prob(\ccalE_1) 
    &= 
    \Prob(\left\{Z(\theta) \geq 0
    \text{ and }
    Z(\theta^*) \geq 0
    \right\} ) \\
    &\geq
    \Prob(\left\{Z(\theta) \geq \text{RHS of \eqref{eq: Z(theta) positive}} \right\}) \\
    &\geq
    1 - 
    2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right).
\end{align}
%%%%
\fi
Now, define
%%%%
\begin{gather}
    \ccalE_2 = 
    \left\{
    |Z(\theta) - Z(\theta^*)| 
    \leq 
    3n \| \theta^* \| \| \theta - \theta^* \|
    \right\}
\end{gather}
%%%%
We have that
%%%%
\begin{align} 
    Z(\theta) - Z(\theta^*)
    =
    \sum_{i=1}^{n} \langle X_i, \theta - \theta^* \rangle Y_i
    =
    \sum_{i=1}^{n} \langle X_i, \theta - \theta^*\rangle \langle X_i, \theta^*\rangle 
    +
    \sum_{i=1}^{n} \langle X_i, \theta - \theta^*\rangle \epsilon_i
\end{align}
%%%%
From Lemma \ref{lemma: sub-exponential}, we have
%%%%
\begin{align} 
    \sum_{i=1}^{n} \langle X_i, \theta - \theta^*\rangle \langle X_i, \theta^*\rangle 
    \sim
    \SubE(4 \| \theta^* \|^2 \| \theta - \theta^* \|^2, 4 \| \theta^* \| \| \theta - \theta^* \|)
\end{align}
%%%%
Therefore, with probability at least $1 -  2 \exp(-n/8)$,
%%%%
\begin{gather}
    \bigg| \sum_{i=1}^{n} \langle X_i, \theta - \theta^*\rangle \langle X_i, \theta^*\rangle - n \langle  \theta - \theta^*, \theta^*\rangle \bigg|
    \leq
    n \| \theta^* \| \| \theta - \theta^* \|,
\end{gather}
%%%%
implying that
%%%%
\begin{gather}
    \bigg| \sum_{i=1}^{n} \langle X_i, \theta - \theta^*\rangle \langle X_i, \theta^*\rangle \bigg|
    \leq
    n |\langle  \theta - \theta^*, \theta^*\rangle|
    +
    n \| \theta^* \| \| \theta - \theta^* \|
    \leq
    2n \| \theta^* \| \| \theta - \theta^* \|.
\end{gather}
%%%%
On the other hand,
%%%%
\begin{align} 
    \sum_{i=1}^{n} \langle X_i, \theta - \theta^*\rangle \epsilon_i
    \sim
    \SubE\left(\frac{n\| \theta - \theta^* \|^2 \sigma^2}{2}, \| \theta - \theta^* \| \sigma \right)
\end{align}
%%%%
Therefore,
%%%%
\begin{gather}
    \bigg|\sum_{i=1}^{n} \langle X_i, \theta - \theta^*\rangle \epsilon_i \bigg|
    \leq
    n \| \theta - \theta^* \| \| \theta^* \|,
\end{gather}
%%%%
with probability at least
%%%%
\begin{align}
    1 - 2 \exp\left( -  n \min\left\{ \SNR^2
    ,
    \frac{\SNR}{2} \right\}\right).
\end{align}
%%%%
Therefore,
%%%%
\begin{align} 
    \Prob(\ccalE_2) 
    =
    \Prob(\left\{
    |Z(\theta) - Z(\theta^*)| 
    \leq 
    3n \| \theta^* \| \| \theta - \theta^* \|
    \right\})
    \geq
    1 - 
    2 \exp\left( -\frac{n}{8} \right)
    -
    2 \exp\left( -  n \min\left\{ \SNR^2
    ,
    \frac{\SNR}{2} \right\}\right).
\end{align}
%%%%
Putting all together,

%%%%
\begin{align} 
    \Prob(\ccalE) 
    &=
    \Prob(\ccalE_1 \cap \ccalE_2) \\
    &\geq
    1 - 
    2 \exp\left( -\frac{n}{32} \left( \frac{1-\alpha}{1+\alpha}\right)^2\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \left( \frac{1 - \alpha}{1 + \alpha}\right)^2 \SNR^2
    ,
    \frac{1}{8} \left( \frac{1 - \alpha}{1 + \alpha}\right) \SNR \right\}\right) \\
    &\quad - 
    2 \exp\left( -\frac{n}{32}\right)
    -
    2 \exp\left( -  n \min\left\{ \frac{1}{16} \SNR^2
    ,
    \frac{1}{8} \SNR \right\}\right) \\
    &\quad-
    2 \exp\left( -\frac{n}{8} \right)
    -
    2 \exp\left( -  n \min\left\{ \SNR^2
    ,
    \frac{\SNR}{2} \right\}\right)
\end{align}
%%%%






\end{proof}
%%%%
